Towards Automated Design of Bayesian Optimization via Exploratory Landscape Analysis

Bayesian optimization (BO) algorithms form a class of surrogate-based heuristics, aimed at efficiently computing high-quality solutions for numerical black-box optimization problems. The BO pipeline is highly modular, with different design choices for the initial sampling strategy, the surrogate model, the acquisition function (AF), the solver used to optimize the AF, etc. We demonstrate in this work that a dynamic selection of the AF can benefit the BO design. More precisely, we show that already a na\"ive random forest regression model, built on top of exploratory landscape analysis features that are computed from the initial design points, suffices to recommend AFs that outperform any static choice, when considering performance over the classic BBOB benchmark suite for derivative-free numerical optimization methods on the COCO platform. Our work hence paves a way towards AutoML-assisted, on-the-fly BO designs that adjust their behavior on a run-by-run basis.

==> figure1.tex <==
\begin{figure}[ht]
\begin{floatrow}
\ffigbox{%
  \includegraphics[width=0.48\textwidth]{figures/convergence/regret_over_steps_dimension_5.pdf}
}{%
  \caption{Switching \ac{AF}s and especially selecting \ac{AF} schedules (\ac{AFS}) is beneficial. Scaled log-regret averaged over \num{5} instances of all \num{24} BBOB functions for \num{5} dimensions with the \SI{95}{\percent} confidence interval for the schedules from~\cref{tab:schedules}.}
    \label{fig:convergence_all_ci}
} \quad
\ffigbox{%
 \includegraphics[width=.48\textwidth]{figures/histogram/perbbob_dimension_5-function_4_2x4.pdf}
}{
\caption{Ranks of schedules for BBOB function 4.}
    \label{fig:rank}
    }
%\capbtabbox{%
%\resizebox{0.48\textwidth}{!}{
%    \begin{tabular}{ll}
%        \toprule
%         Name & Schedule \\
%         \midrule
%         static (EI) & \includegraphics[width=3cm]{figures/schedules/ei.png}\\
%         static (PI) & \includegraphics[width=3cm]{figures/schedules/pi.png}\\
%         random & \includegraphics[width=3cm]{figures/schedules/random.png}\\
%         round robin & \includegraphics[width=3cm]{figures/schedules/roundrobin.png}\\
%         explore-exploit (\num{0.25}) & \includegraphics[width=3cm]{figures/schedules/exex25.png}\\
%         explore-exploit (\num{0.5}) & \includegraphics[width=3cm]{figures/schedules/exex50.png}\\
%         explore-exploit (\num{0.75}) & \includegraphics[width=3cm]{figures/schedules/exex75.png}\\
%         VBS \small{(Virtual Best Solver)} &
%         \includegraphics[width=3cm]{figures/schedules/vbs.png}\\
%         AFS \small{(\ac{AF} Selector)}&
%         \includegraphics[width=3cm]{figures/schedules/afs.png}\\
%        %   Virtual Best Solver \\
%        %  AFS & Selected AF Schedule \\
%         \bottomrule
%    \end{tabular}
%    }
%}
%{%
%  \caption{Schedule portfolio of PI, EI and their combinations. AFS is a selector that aims to predict which of the first seven schedules is the best. VBS is a perfect selector and forms the ground truth for AFS.}%
%  \label{tab:schedules}
%}
\end{floatrow}
\end{figure}
